EVOR: Evolving Retrieval for Code Generation

Recently the retrieval-augmented generation (RAG) has been successfully applied in code generation. However, existing pipelines for retrieval-augmented code generation (RACG) employ static knowledge bases with a single source, limiting the adaptation capabilities of Large Language Models (LLMs) to domains they have insufficient knowledge of. In this work, we develop a novel pipeline, EVOR, that employs the synchronous evolution of both queries and diverse knowledge bases. On two realistic settings where the external knowledge is required to solve code generation tasks, we compile four new datasets associated with frequently updated libraries and long-tail programming languages, named EVOR-BENCH. Extensive experiments demonstrate that EVOR achieves two to four times of execution accuracy compared to other methods such as Reflexion (Shinn et al., 2024), DocPrompting (Zhou et al., 2023), etc. We demonstrate that EVOR is flexible and can be easily combined with them to achieve further improvement. Further analysis reveals that EVOR benefits from the synchronous evolution of queries and documents and the diverse information sources in the knowledge base. We hope that our studies will inspire more insights into the design of advanced RACG pipelines in future research. Our model, code, and data are available at https://arks-codegen.github.io.

==> tables/active_retrieval.tex <==
\begin{table}[t]
\centering
\small
\scalebox{0.9}{
\begin{tabular}{ccccccc}
\toprule
Retrieval & \newscience & Tensor-M & Ring & Pony & Avg   \\
\midrule
 \multicolumn{6}{c}{\textit{Model: ChatGPT}} \\
 No Retrieval & 17.6 & 11.1 & 3.7 & 1.8 & 8.6\\
 One-Time Retrieval & 32.4  & 33.3  & 8.4 & 2.7 & 19.2\\
 Active Retrieval & 37.3  & 53.3  & 35.5 & 12.4 & 34.6\\
\midrule
 \multicolumn{6}{c}{\textit{Model: CodeLlama}} \\
  No Retrieval & 11.3 & 17.8 & 0.0 & 0.0 & 7.3 \\
  One-Time Retrieval & 16.9 & 37.8 & 4.7 & 4.4 & 16.0\\
  Active Retrieval & 30.3 & 51.1 & 26.2 & 16.8 & 31.1\\
\bottomrule
\end{tabular}
}
\caption{\label{tab:active_retrieval}The comparison of LLM performance without retrieval (None Retrieval), One-Time Retrieval, and Active Retrieval from the diverse knowledge soup (execution feedback, code snippets, and documentation). 
Tensor-M denotes \jumptensor. 
The significant improvement enhanced by active retrieval implies the necessity for LLMs to iteratively refine the query and interact with the knowledge soup in generalized code generation.
}
\end{table}

==> tables/iterative_learning.tex <==
\begin{table}
\centering
\small
\begin{tabular}{ccccccc}
\hline
 \multicolumn{3}{l}{\textbf{Model: ChatGPT}} \\
\hline
Knowledge & \newscience & Tensor-M & Ring & Pony & Avg   \\
\hline
 None & 17.6 & 11.1 & 3.7 & 1.8 & 8.6\\
 Doc & 32.4  & 33.3  & 8.4 & 2.7 & 19.2\\
 Doc$_I$ & 35.2  & 48.9  & 26.7 & 5.3 & 29.0\\
 Code & 21.8  & 20.0  & 7.5 & 4.4 & 13.4\\
 Code$_I$ & 28.2  & 31.1  & 24.3 & 7.1 & 22.7\\
\hline
 \multicolumn{3}{l}{\textbf{Model: CodeLlama}} \\
\hline
  None & 11.3 & 17.8 & 0.0 & 0.0 & 7.3 \\
  Doc & 16.9 & 37.8 & 0.9 & 4.4 & 15.0\\
  Doc$_I$ & 26.1  & 44.4 & 0.9 & 10.6 & 20.5\\
  Code & 14.8 & 26.7 & 4.7 & 7.1 & 13.3\\
  Code$_I$ & 17.6  & 35.6 & 26.2 & 15.9 & 23.8\\
\hline
\end{tabular}
\caption{\label{tab:iterative_learning}The comparison of single-round generation and iterative learning of LLM on code snippets and documentation. Tensor-M denotes \jumptensor, Code denotes Code snippets, Doc denotes the documentation and the subscript $I$ denotes applying the iterative learning on the knowledge source. The results demonstrate the significant improvement of iterative learning, which implies the necessity for LLM to iteratively learn from knowledge sources in writing generalized code.
}
\end{table}

==> tables/knowledge.tex <==
\begin{table}
\centering
\small
\begin{tabular}{lcc}
\toprule
% \cmidrule{2-6}
% \cmidrule{8-12}
Knowledge ($\downarrow$) & ChatGPT  & CodeLlama \\
\midrule
None & 8.6 & 7.3\\
\midrule
\multicolumn{3}{c}{\textit{Single Source Retrieval}} \\
Web & 9.7 & 7.5\\
Exec & 12.6 & 7.6\\
Code & 22.7 & 23.8\\
Doc & 28.9 & 20.5 \\
\midrule
\multicolumn{3}{c}{\textit{Knowledge Soup Retrieval}} \\
Exec + Code & 27.1 & 24.0 \\
Exec + Doc & 31.0 & 21.5\\
Code + Doc & 32.4 & 30.6\\
Exec + Code + Doc & \textbf{34.6} & \textbf{31.1}\\
\bottomrule
\end{tabular}
\caption{The average performance of ChatGPT and CodeLlama with different knowledge sources. The results show that diverse types of knowledge enhance RACG performance for both ChatGPT and CodeLlama.\label{table:knowledge}
}
\end{table}



==> tables/main.tex <==
\begin{table*}
\centering
\small
\begin{tabular}{lc ccccc c ccccc}
\toprule
\textbf{Knowledge} & & \multicolumn{5}{c}{\textbf{Model: ChatGPT}} & & 
\multicolumn{5}{c}{\textbf{Model: CodeLlama}}\\
% \cline{1-1}
\cmidrule{3-7}
\cmidrule{9-13}
 & & \newscience & Tensor-M & Ring & Pony & Avg. & & \newscience & Tensor-M & Ring & Pony  & Avg. \\
% \cline{1-5}
% \cline{7-11}
% \cline{1-1}
% \cline{3-7}
% \cline{9-13}
\midrule
None & & 17.6 & 11.1 & 3.7 &  1.8 & 8.6 & & 11.3 & 17.8 & 0.0 & 0.0 & 7.3\\
% \cline{1-1}
% \cline{3-7}
% \cline{9-13}
\midrule
\multicolumn{13}{c}{\textit{Single Source Retrieval (Baseline)}} \\
% \hline
Web & & 19.0 & 13.3 & 4.7 & 1.8 & 9.7 & & 12.0 & 17.8 & 0.0 & 0.0 & 7.5\\
Exec & & 21.1 & 20.0 & 4.7 &  4.4 & 12.6 &  & 12.7 & 17.8 & 0.0 &  0.0 & 7.6\\
Code & & 28.2 & 31.1 & 24.3 & 7.1 & 22.7 &  & 17.6 & 35.6 & 26.2 &  15.9 & 23.8\\
Doc & & 35.2 & 48.9 & 26.2 & 5.3 & 28.9 &  & 26.1 & 44.4 & 0.9 & 10.6 & 20.5 \\
% Gold Doc & & 37.3 & 51.1 & 28.0 & 5.3 & 30.4 & & 27.5 & 46.7 & 1.9 & 12.4 & 22.1 \\
% \cline{1-1}
% \cline{3-7}
% \cline{9-13}
\midrule
\multicolumn{13}{c}{\textit{Knowledge Soup Retrieval (Ours)}} \\
Exec + Code & & 33.1 & 40.0 & 26.2 &  8.9 & 27.1 &  & 18.4 & 35.6 & 26.2 & 15.9 & 24.0 \\
Exec + Doc & & 36.6 & 53.3 & 27.1 &  7.1 & 31.0 & & 26.8 & 46.7 & 0.9 &  11.5 & 21.5\\
Doc + Code & & 37.3 & 48.9 & 34.6 &  8.9 & 32.4 &  & 30.3 & 48.9 & 26.2 &  16.8 & 30.6\\
% \cline{1-1}
% \cline{3-7}
% \cline{9-13}
Doc + Code + Exec & & \textbf{37.3} & \textbf{53.3} & \textbf{35.5} & \textbf{12.4} & \textbf{34.6} & & \textbf{30.3} & \textbf{51.1} & \textbf{26.2} & \textbf{16.8} & \textbf{31.1}\\
\bottomrule
%Gold Documents + Error messages + Code snippets &  &  &  &  &  \\
%\hline
\end{tabular}

\caption{\label{table:main}ChatGPT and CodeLlama execution accuracy with different knowledge sources. 
Tensor-M refers to \jumptensor and Avg. refers to the average score across four benchmarks. 
Web denotes the web search content; 
Exec denotes the execution feedback from compiler/interpreter; 
Code denotes the code snippets generated by LLMs in previous rounds that are verified to be free of syntax error; 
Doc refers to the documentation. 
% Including all of the documentation, execution feedback, and code snippets consistently gives the best performance across the four benchmarks.
Adding more knowledge sources consistently enhances the performance, which demonstrates the advantage of a diverse knowledge soup in the RACG pipeline.
}
\end{table*}

% \begin{table}
% \centering
% \begin{tabular}{lccccc}
% \hline
%  \multicolumn{3}{l}{\textbf{Model: CodeLlama}} \\
% \hline
% Knowledge & \newscience & \jumptensor & Ring & Pony   \\
% \hline
% None & 11.3 & 17.8 & 0.0 & 0.0   \\
% \hline
% Google & 12.0 & 17.8 & 0.0 & 0.0   \\
% EF & 12.7 & 17.8 & 0.0 &  0.0  \\
% CS & 17.6 & 35.6 & 26.2 &  15.9  \\
% D & 26.1 & 44.4 & 0.9 & 10.6   \\
% \hline
% EF + CS & 17.6 & 35.6 & 26.2 & 15.9   \\
% EF + D & 26.8 & 46.7 & 0.9 &  11.5  \\
% D + CS & 30.3 & 48.9 & 26.2 &  16.8 \\
% \hline
% D + CS + EF & \textbf{30.3} & \textbf{51.1} & \textbf{26.2} & \textbf{16.8}  \\
% \hline
% %Gold Documents + Error messages + Code snippets &  &  &  &  &  \\
% %\hline
% \end{tabular}
% \label{table:main}
% \caption{CodeLlama execution accuracy when different knowledge sources are used. Including all of documents, error messages, and code snippets consistently generates the best performance across the four benchmarks.
% }
% \end{table}

==> tables/open_source_model.tex <==
\begin{table*}
\centering
\begin{tabular}{ccccccc}
\hline
Model & Knowledge source & NewScience & Jumptensor & Ring & Pony & Average   \\
\hline
 & None &  &  &  &  &  \\
 & Google search &  &  &  &  &  \\
StaCoder(15B) & Error messages &  &  &  &  &  \\
 & Code snippets &  &  &  &  &  \\
 & Documents &  &  &  &  &  \\
\hline
 & None &  &  &  &  &  \\
 & Google search &  &  &  &  &  \\
CodeLlama(34B) & Error messages &  &  &  &  &  \\
 & Code snippets &  &  &  &  &  \\
 & Documents &  &  &  &  &  \\
\hline
 & None &  &  &  &  &  \\
 & Google search &  &  &  &  &  \\
Lemur(70B) & Error messages &  &  &  &  &  \\
 & Code snippets &  &  &  &  &  \\
 & Documents &  &  &  &  &  \\
\hline
 & None & 17.61 & 11.11 &  &  &  \\
 & Google search & 21.83 & 17.78 &  &  &  \\
ChatGPT & Error messages & 21.13 & 20.00 &  &  &  \\
 & Code snippets & 28.17 & 31.11 &  &  &  \\
 & Documents & 35.21 & 44.44 &  &  &  \\
\hline
\end{tabular}
\label{table:open_source_models}
\caption{Experimental results on open-source models. ChatGPT is included for easier comparison.
}
\end{table*}

==> tables/query.tex <==
\begin{table}
\centering
\small
\begin{tabular}{ccccccc}
\hline
 \multicolumn{3}{l}{\textbf{Model: ChatGPT}} \\
\hline
Retrieval & \newscience & Tensor-M & Ring & Pony & Avg   \\
\hline
 None & 17.6 & 11.1 & 3.7 & 1.8 & 8.6\\
 Non-Active & 32.4  & 33.3  & 8.4 & 2.7 & 19.2\\
 Active & 37.3  & 53.3  & 35.5 & 12.4 & 34.6\\
\hline
 \multicolumn{3}{l}{\textbf{Model: CodeLlama}} \\
\hline
  None & 11.3 & 17.8 & 0.0 & 0.0 & 7.3 \\
  Non-Active & 16.9 & 37.8 & 4.7 & 4.4 & 16.0\\
  Active & 30.3 & 51.1 & 26.2 & 16.8 & 31.1\\
\hline
\end{tabular}
\caption{\label{tab:query_formulation}
}
\end{table}

==> tables/retrieval_acc.tex <==
\begin{table}
\centering
\small
\begin{tabular}{ccccccc}
\midrule
 & \newscience & Tensor-M & Ring & Pony & Average   \\
\midrule
 BM25-R & 42.3 & 45.6 & 9.4 & 7.8 & 26.3 \\
 BM25-G & 31.0 & 31.1 & 5.6 & 3.5 & 17.8 \\
 INST-R & 62.7 & 71.1 & 56.1 & 48.7 & 59.7 \\
 INST-G & 37.3 & 53.3 & 35.5 & 12.4 & 34.6 \\
 text-R & 66.2 & 77.8 & 63.6 & 52.2 & 65.0\\
 text-G & 38.7 & 55.6 & 36.4 & 13.3 & 36.0\\
 SFR-R & 69.1 & 77.8 & 59.8 & 54.0 & 65.2\\
 SFR-G & 39.4 & 55.6 & 37.4 & 14.2 & 36.7\\
\midrule
\end{tabular}
\caption{\label{tab:retrieval_acc}The retrieval accuracy (percentage of examples where all the gold documentation has been retrieved, denoted as "-R") and generalization performance ("-G") of ChatGPT when BM25, INSTRUCTOR (INST), text-embedding-3-large (text) or SFR-Embedding-Mistral (SFR) is used as the retrieval model. 
There is a big gap between the two accuracies, indicating that in a lot of cases, even if the gold documentation is included in the prompt, ChatGPT still fails to generate the correct code.}
\end{table}






==> tables/swe.tex <==
\begin{table}[t]
\centering
\small
\scalebox{0.95}{
\begin{tabular}{cccccc}
\toprule
Method & RAG & \ourmethod & Agent & Agent+\ourmethod   \\
\midrule
 GPT-4 & 2.7 & 17.3 & 18.0 & 19.3\\
 Claude-3 & 4.3 & 12.0 & 11.7 & 13.3\\
\bottomrule
\end{tabular}
}
\caption{Performance of RAG, \ourmethod, SWE-agent (Agent) and combination of \ourmethod and SWE-agent. The numbers are shown in the rate of resolved issues in SWE-bench-Lite.\label{tab:swe}
}
\end{table}

==> texts/abstract.tex <==
%     \begin{abstract}
% Recent progress in large language models (LLM) has shown its notable capacity to write codes. 
% However, it remains unclear what helps LLM to generalize and write codes they have not seen during training.
% In this study, we investigate this problem from multiple perspectives, including retrieval-augmented generation, long-context modeling, iterative learning and etc.  
% We conduct extensive experiments on four datasets, where two require LLM to write codes from rare programming languages Pony and Ring, and two require LLM to write codes from updated Python libraries.
% Our analysis reveals that: 1). the design of query and documentation significantly affects the quality of retrieval and code generation; 2). naively including more documentation may not boost the performance; 3). LLM learns external knowledge during the iterative process 3). apart from documentation, LLM can also learn from other sources (e.g., code snippets) and the self-debugging process.
% Built on that, we further introduce an innovative paradigm that significantly improves LLM's generalization ability by xxx\%.
% Our code will be released at: xxx.
% \end{abstract}


\begin{abstract}
% Large language models (LLMs) such as ChatGPT and Codex have exhibited incredible proficiency in code generation.
% However, they struggle with out-of-domain code generation, which deviates from their pretraining data.
% Given their strong capabilities to incorporate external knowledge in test time, we explore the paradigm for effective LLMs generalized code writing.
% Specifically, we compare four knowledge sources that LLMs can potentially utilize for adaptation: documentation, web content, execution feedback, and code snippets.
% We then investigate the pipelines for LLMs to effectively leverage external knowledge. 
% Finally, we introduce a new benchmark consisting of four datasets that reflect realistic generalization scenarios: coding in updated libraries and long-tail programming languages.
% % Next, we compare four knowledge sources that LLM can potentially utilize for adaptation.
% % Furthermore, we investigate the pipelines for LLM to effectively leverage external knowledge.
% Our experiments demonstrate that (1). all of the four proposed knowledge sources enhance LLMs generalization performance, among which documentation and code snippets are the most effective; (2). with combinatorial knowledge sources and carefully designed pipelines, ChatGPT and CodeLlama improve the average execution accuracy by 26.5\% and 23.8\% respectively.
% We conduct extensive experiments and detailed analysis and provide rich insights into understanding the task of generalizing LLMs in code writing.
% Our code and data are available at anonymized.
% \qian{Recently the topic of retrieval-augmented generation (RAG) on text corpus become more and more popular. The paradigm is usually regarded as the most promising way to incorporate external knowledge to the model without training. However, applying RAG on code generation is still under-explored. In this paper, we investigate the line of retrieval-augmented code generation, and try to answer the key challenge of what, how and when to retrieve. Specifically, we propose to leverage four kinds of knowledge LLMs can potentially retrieve: documentation, web content, execution feedback, and code snippets. Then, regarding for how, we argue that task description is not the optimal way to retrieve. As for when, we propose an iterative method to retrieve multiple times to empower the model to improve itself iteratively. To benchmark the system, we collect a new benchmark which requires external knowledge to answer realistic questions regarding libraries or programming languages. Experimental results demonstrate that our pipeline improves the average execution accuracy of powerful code generation models by a large margin. The analysis show that all of our proposed improvements on what, how and when are very effective for RACG.}
% \qian{
Recently the retrieval-augmented generation (RAG) paradigm has raised much attention for its potential in incorporating external knowledge into large language models (LLMs) without further training.
% Specific to code generation, the frequently updated libraries and customized programming languages in the industry inherently require LLMs to generalize efficiently.
While widely explored in natural language applications, its utilization in code generation remains under-explored.
In this paper, we introduce Active Retrieval in Knowledge Soup (\ourmethod), an advanced strategy for generalizing large language models for code.
%, with a focus on tackling the challenges associated with what to retrieve and how to retrieve.
In contrast to relying on a single source, we construct a knowledge soup integrating web search, documentation, execution feedback, and evolved code snippets.
%, serving as an effective corpus for code generation.
We employ an active retrieval strategy that iteratively refines the query and updates the knowledge soup.
% Our proposed approach is designed for seamless integration with any existing code generation model.
To assess the performance of \ourmethod, we compile a new benchmark comprising realistic coding problems associated with frequently updated libraries and long-tail programming languages.
Experimental results on ChatGPT and CodeLlama demonstrate a substantial improvement in the average execution accuracy of \ourmethod on LLMs. 
The analysis confirms the effectiveness of our proposed knowledge soup and active retrieval strategies, offering rich insights into the construction of effective retrieval-augmented code generation (RACG) pipelines.
\end{abstract}

\vspace{-2pt}

==> texts/intro.tex <==

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/figure1_v5.pdf}
    \caption{Instead of depending solely on human instructions for knowledge soup retrieval and completing the pipeline in a single round, we actively engage in the retrieval process through the following steps: (1) generating code and updating the knowledge soup; (2) refining the query; (3) retrieving information from the knowledge soup and back to (1). Through active retrieval for N iterations, both the query and knowledge soup undergo improvements, ultimately enhancing the quality of the generated code.}
    \label{fig:main}
\end{figure}


% \begin{figure*}[ht]
% % \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=2\columnwidth]{figures/figure1.pdf}}
% \caption{Instead of directly using the natural language question to retrieve documentation and finishing the retrieval-augmented generation in just a single round (orange pipeline), we actively continue the retrieval process by: (1). formulating the query with the question, code output, execution feedback, and the explained code generated by LLM; (2). retrieving from diverse knowledge sources including documentation, code snippets, execution feedback and web content (blue pipeline). The code snippets are dynamically updated with new code outputs verified to be free of syntax error. With active retrieval, both query and knowledge sources are improved in each iteration, which finally enhances LLM generation quality.}
% \label{fig:main}
% \end{center}
% \vskip -0.4in
% \end{figure*}
\section{Introduction}

% Introduce RAG and why it should be introduced in code generation (@Shuyan's paper can be a good reference, compare to Daoguang's paper on continual pre-training)
The retrieval-augmented generation (RAG) paradigm has raised significant attention in the era of large language models (LLMs)~\citep{guu2020realm,karpukhin-etal-2020-dense,izacard2023atlas,borgeaud2022retro,retrieval-lm-tutorial}. It empowers LLMs to effectively assimilate external knowledge~\citep{khattab2022dsp}, providing reference~\citep{menick2022teaching}, and boosting overall performance~\citep{jiang-etal-2023-active}.
% By enabling LLMs to read and incorporate information from external knowledge, this paradigm represents a promising avenue to inject domain knowledge, especially on unseen or long-tailed domains to LLMs without additional training [citation].
% Although it's important, it is not well explored in the literature. (Cite most related works and introduce the two aspects we want to improve in the following)
While the realm of text-based applications has witnessed extensive advancements in RAG over the years, the progress in retrieval-augmented code generation (RACG) has not kept pace with that of language applications~\citep{zhou2023docprompting,zhang-etal-2023-repocoder}.
This may be partially attributed to the fact that existing LLMs have already shown strong abilities in code generation~\citep{chen2021evaluating,hendrycks2021measuring,li2022competition,fried2022incoder,xu2022systematic,li2023starcoder}.
Unlike textual corpora, which tends to be consistently stable, code repositories undergo frequent updates, which often encompass modifications aimed at disabling undesirable functions, the integration of new features, and the introduction of fresh syntactic sugar~\cite{tsql,ali2023x,bugden2022rust}.
Considering the dynamic nature of code, it is crucial to tackle the challenges in RACG.
% Meanwhile, new programming languages with distinct grammatical rules continue to emerge, on which LLMs may not be sufficiently trained to be adequately proficient\cite{tsql,ali2023x,bugden2022rust}.

% Our method, how to improve and cue Figure 1 there
Building on the success of practices in RAG, earlier efforts on RACG have primarily centered around generating code through retrieval from the web content (e.g., Stack Overflow)~\citep{parvez-etal-2021-retrieval-augmented,wang2022execution}, the code documentations~\citep{zan2022language,zhou2023docprompting}, or the source code in the same repository~\citep{zhang-etal-2023-repocoder,shrivastava2023repofusion}.
% Previous works mainly focus on code generation via retrieving from code documentations~\citep{zhou2023docprompting}, or retrieves relevant code from a predefined database~\citep{parvez-etal-2021-retrieval-augmented}, 
% They have demonstrated that retrieving relevant documentation is essential to help LLM generalize to unseen function calls.
% For example, when a compiler produces an error message for an incorrect code, leveraging that message to conduct a web search can lead to the discovery of a solution page. Language Models (LLMs) can then utilize this information to generate accurate and context-aware code. 
% Despite their effectiveness, we argue that retrieval from single source is not the optimal choice, particularly because we regard code generation as a more like multi-hop process. For example, when a compiler detects a syntax error in the generated code, utilizing the error message to initiate a web search can uncover a pertinent coding example.
While these approaches have proven effective for code generation, they generally treat it as a one-time process and only employ a single-source (i.e., either documents or code) for retrieval.
% However, we argue that a single-source retrieval may not always be the most optimal choice, particularly when considering code generation as a multi-hop process. For example, when the compiler identifies a syntax error for the generated code, leveraging the error message to initiate a web search can unveil relevant coding examples.
% This example motivates us to think of a more dynamic and active exploration of potential solutions, facilitating the code generation process.
However, we argue that exclusively relying on single-source retrieval may not be the optimal choice , especially in the context of code generation.
For example, when the compiler identifies a syntax error for the generated code, leveraging the error message to initiate a web search can unveil relevant coding examples.
LLMs can then utilize such information to generate code with higher quality.
% For example, compelling scenario supporting our argument arises when a compiler detects a syntax error in the generated code. In such cases, leveraging the error message to initiate a web search may reveal pertinent coding examples. 

Motivated by the above example, in this paper, we posit that RACG should be conceptualized as a multi-round process with active exploration. Specifically, we advocate for a more active retrieval of all available information we can leverage, which we use ``knowledge soup'' to note in the below.
The knowledge soup here includes the web content from the search engine, the related documentation, the feedback from code execution, and the dynamically added code snippets.
Different from single-source, these different information build the multi-source retrieval pipeline, which facilitate the diversity of the retrieved information during code generation.
Meanwhile, as depicted in Figure~\ref{fig:main}, \ourmethod leverages a multi-round procedure which generates and retrieves information iteratively.
Different from the traditional single-round code generation, our retrieval process stands out as both the query and the knowledge soup undergo continuous updates after each iteration. This strategic refinement aims to facilitate the recall of more pertinent information. 
Through multiple-round interactions with the knowledge soup, the LLM progressively improves the generated code.


% can be much better with multi-source retrieval, which we use ``knowledge soup'' to represent in the below.
% In this paper, we argue that existing efforts for RACG may not be enough, especially those experience from text-based applications.
% We explore very different strategies.
% Build a benchmark, conduct experiments and achieve a great performance. Summarize the contributions
To evaluate our system in the generalization setting with LLMs pre-trained on massive public data, we propose a novel benchmark comprising four datasets designed to simulate updates in code repositories. Specifically, two of these datasets focus on modifications made to widely-used Python libraries, Scipy and Tensorflow. The remaining two datasets simulate the introduction of new grammars, with the help of two less-common programming languages Ring and Pony.
% Our method is theoretically integrated with various LLMs good at coding.
To conduct thorough experiments, we employ both proprietary models, such as ChatGPT, and open-source models like CodeLlama~\citep{roziere2023code}.
Experimental results across these four datasets demonstrate that our method can yield a significant improvement in the average performance of different LLMs.
For example, on the Ring dataset, our method showcases an impressive boost, elevating the performance of ChatGPT from $3.7$\% to $35.5$\%. 
The further analysis unveils an unexpected finding: web search, the most widely utilized method in RAG, is not as effective as expected.
In contrast, the effectiveness of RACG is notably influenced by code snippets, code documentation, and execution feedback.
% Remarkably, our observations indicate that LLMs tend to derive more effective generation from code snippets compared to code documentations.
Finally, we showcase the notable advancements attained through our active retrieval approach, demonstrating an improvement of up to $27.1$\% when compared to the results achieved through single-round retrieval.
We will release the code and the new benchmark upon acceptance.

% For example, on the Ring dataset, our method can boost ChatGPT from 3.7\% to 35.5\%.
% Further analysis reveals that, surprisingly web search, the widely used retrieval method in RAG, is not as effective as expected. In contrast, the code snippets, the code documentations and the execution feedback all play a pivotal role in boosting the performance of RACG.
% Notably, LLMs often derive more effective learning from code snippets than from code documentations. 
% Last, we present the significant improvement achieved by iterative learning, which can be up to 21.5\% compared to the results in the first-round generation.

% show that varying ways of crafting queries can cause up to a 19.7\% variation, and different retrieval models can result in up to 20.6\% difference in the final code generation performance.

% (a). To avoid data leakage, we modify two popular Python libraries Scipy and Tensorflow to simulate real updates; (b). We curate Leetcode questions and require LLMs to write code using two long-tail programming languages, Ring and Pony.
% We demonstrate that besides documentation, code snippets are also an important resource for LLM generalization.
% In particular, language models that focus on code such as CodeLlama often find code snippets to be a more effective resource for learning compared to the official documentation.
% Moreover, we notice the synergistic benefits of combining documentation and code snippets, which significantly improve the generalization capabilities of LLMs.


% build a new benchmark on top of DS1000 [citation], and build the dataset for models.

% We experiment with both sparse retrievers such as BM25 and dense retrievers such as INSTRUCTOR.
% To understand the relationship between retrievers and long-context models, we compare the generalization performance with maximum 4k, 8k, 12k, and 16k context windows.
% In contrast to simple prompting or traditional retrieval-augmented generation (RAG), we investigate whether LLMs benefit from iterative learning from knowledge sources.
% As opposed to single-round generation, the query is iteratively updated to retrieve potentially more relevant information, and LLM gradually improves itself in multiple-round interactions with knowledge sources.
% Finally, we introduce a new benchmark of four datasets to evaluate LLMs generalization performance in coding: (a). To avoid data leakage, we modify two popular Python libraries Scipy and Tensorflow to simulate real updates; (b). We curate Leetcode questions and require LLMs to write code using two long-tail programming languages, Ring and Pony.

% We conduct comprehensive experiments with both proprietary models (ChatGPT) and open-source models (CodeLlama). 
% We demonstrate that besides documentation, code snippets are also an important resource for LLM generalization.
% In particular, language models that focus on code such as CodeLlama often find code snippets to be a more effective resource for learning compared to the official documentation.
% Moreover, we notice the synergistic benefits of combining documentation and code snippets, which significantly improve the generalization capabilities of LLMs.
% Across four datasets, we notice that varying ways of crafting queries can cause up to a 19.7\% variation, and different retrieval models can result in up to 20.6\% difference in LLM generalization performance.
% This highlights the importance of retrieval design in LLM generalization pipelines.
% Last but not least, we present the significant improvement achieved by iterative learning, which can be up to 21.5\% compared to the results in the first-round generation.
% Given the expensive computational costs in iterative generation, we conduct a detailed analysis by investigating the relationships between LLMs generalization performance and the number of tokens LLMs process.
% Upon publication, we will release our code and new benchmarks, including annotation of oracle documents and ground-truth code solutions for each example, together with pools of documentation, to serve as a test-bed for future research on updated libraries and long-tail programming languages.


% Distinct from these recent efforts, we comprehensively investigate the paradigm of LLM generalized code writing.
% Specifically, we first compare four knowledge sources that human programmers frequently refer to: Documentation, web content, execution feedback, and code snippets. 
% We analyze the effectiveness of each source and the advantage of their interactions in enhancing LLMs generalization.
% We retrieve one or more knowledge sources and concatenate them with problem descriptions, conditioning on which, LLMs are expected to generalize code writing.
% Furthermore, we investigate the pipelines for LLMs to effectively utilize external knowledge.
% We explore several query formulations including using the natural language question, execution feedback, LLM-generated code, or the explained code as queries.
% We experiment with both sparse retrievers such as BM25 and dense retrievers such as INSTRUCTOR.
% To understand the relationship between retrievers and long-context models, we compare the generalization performance with maximum 4k, 8k, 12k, and 16k context windows.
% In contrast to simple prompting or traditional retrieval-augmented generation (RAG), we investigate whether LLMs benefit from iterative learning from knowledge sources.
% As opposed to single-round generation, the query is iteratively updated to retrieve potentially more relevant information, and LLM gradually improves itself in multiple-round interactions with knowledge sources.
% Finally, we introduce a new benchmark of four datasets to evaluate LLMs generalization performance in coding: (a). To avoid data leakage, we modify two popular Python libraries Scipy and Tensorflow to simulate real updates; (b). We curate Leetcode questions and require LLMs to write code using two long-tail programming languages, Ring and Pony.


% To study the generalization problem in code generation, recent works curated benchmarks from private libraries \cite{zan2022language}, machine learning repositories \cite{liu2023ml}, and open-domain forums \cite{wang2022execution}. 
% However, none of them features updated libraries or long-tail programming languages, which reflect realistic scenarios of generalization in code generation. \citet{zhou2023docprompting} demonstrated that retrieving relevant documentation is essential to help LM write unseen function calls. 
% Despite its effectiveness, the documentation, however, is not necessary to be the only optimal resource for generalizing LLM code writing.


% We conduct comprehensive experiments with both proprietary models (ChatGPT) and open-source models (CodeLlama). 
% We demonstrate that besides documentation, code snippets are also an important resource for LLM generalization.
% In particular, language models that focus on code such as CodeLlama often find code snippets to be a more effective resource for learning compared to the official documentation.
% Moreover, we notice the synergistic benefits of combining documentation and code snippets, which significantly improve the generalization capabilities of LLMs.
% Across four datasets, we notice that varying ways of crafting queries can cause up to a 19.7\% variation, and different retrieval models can result in up to 20.6\% difference in LLM generalization performance.
% This highlights the importance of retrieval design in LLM generalization pipelines.
% Last but not least, we present the significant improvement achieved by iterative learning, which can be up to 21.5\% compared to the results in the first-round generation.
% Given the expensive computational costs in iterative generation, we conduct a detailed analysis by investigating the relationships between LLMs generalization performance and the number of tokens LLMs process.
% Upon publication, we will release our code and new benchmarks, including annotation of oracle documents and ground-truth code solutions for each example, together with pools of documentation, to serve as a test-bed for future research on updated libraries and long-tail programming languages.

%%%% Qian Quota


%%%%%%%%%%% Honjin's version %%%%%%%%%%
% Large language models (LLMs) have shown strong abilities in code generation \cite{chen2021evaluating,hendrycks2021measuring,li2022competition,fried2022incoder,xu2022systematic}.
% Given an instruction that expresses a high-level intent, they can accurately write code free of syntax errors.
% However, this proficiency is limited to their familiar domains and they struggle to write code that deviates from their pretraining data.
% % Given the same problem, significant performance degradation is observed when LLM is required to write out-of-domain code.
% Several works have shown significant performance degradation of LLMs in out-of-domain code generation\cite{athiwaratkun2022multi,cassano2022multipl,shrivastava2023repofusion}.


% In real life, numerous software requires LLMs to write code in the designated programming language, on which LLMs may not be sufficiently trained to be adequately proficient\cite{tsql,ali2023x,bugden2022rust}.
% Aside from the new/varied programming language, the generalization problem in code generation naturally arises from updated libraries.
% From time to time, they are modified to disable unfavorable function calls and incorporate new features.
% To be assistive in programming, LLMs are thus required to adaptable and generalizable to keep current with such changes.

% For example, numerous SQL variants are developed by industrial companies (Microsft uses T-SQL and Salesforce uses SOQL), and in 2023, Scipy\footnote{https://pypi.org/project/scipy/#history} was updated 6 times. 

% Most existing work on code generation focuses on in-domain programming, where language models write code seen during training. 

% To study the generalization problem in code generation, recent works curated benchmarks from private libraries \cite{zan2022language}, machine learning repositories \cite{liu2023ml}, and open-domain forums \cite{wang2022execution}. 
% However, none of them features updated libraries or long-tail programming languages, which reflect realistic scenarios of generalization in code generation. \citet{zhou2023docprompting} demonstrated that retrieving relevant documentation is essential to help LM write unseen function calls. 
% Despite its effectiveness, the documentation, however, is not necessary to be the only optimal resource for generalizing LLM code writing.

% Distinct from these recent efforts, we comprehensively investigate the paradigm of LLM generalized code writing.
% Specifically, we first compare four knowledge sources that human programmers frequently refer to: Documentation, web content, execution feedback, and code snippets. 
% We analyze the effectiveness of each source and the advantage of their interactions in enhancing LLMs generalization.
% We retrieve one or more knowledge sources and concatenate them with problem descriptions, conditioning on which, LLMs are expected to generalize code writing.
% Furthermore, we investigate the pipelines for LLMs to effectively utilize external knowledge.
% We explore several query formulations including using the natural language question, execution feedback, LLM-generated code, or the explained code as queries.
% We experiment with both sparse retrievers such as BM25 and dense retrievers such as INSTRUCTOR.
% To understand the relationship between retrievers and long-context models, we compare the generalization performance with maximum 4k, 8k, 12k, and 16k context windows.
% In contrast to simple prompting or traditional retrieval-augmented generation (RAG), we investigate whether LLMs benefit from iterative learning from knowledge sources.
% As opposed to single-round generation, the query is iteratively updated to retrieve potentially more relevant information, and LLM gradually improves itself in multiple-round interactions with knowledge sources.
% Finally, we introduce a new benchmark of four datasets to evaluate LLMs generalization performance in coding: (a). To avoid data leakage, we modify two popular Python libraries Scipy and Tensorflow to simulate real updates; (b). We curate Leetcode questions and require LLMs to write code using two long-tail programming languages, Ring and Pony.

% We conduct comprehensive experiments with both proprietary models (ChatGPT) and open-source models (CodeLlama). 
% We demonstrate that besides documentation, code snippets are also an important resource for LLM generalization.
% In particular, language models that focus on code such as CodeLlama often find code snippets to be a more effective resource for learning compared to the official documentation.
% Moreover, we notice the synergistic benefits of combining documentation and code snippets, which significantly improve the generalization capabilities of LLMs.
% Across four datasets, we notice that varying ways of crafting queries can cause up to a 19.7\% variation, and different retrieval models can result in up to 20.6\% difference in LLM generalization performance.
% This highlights the importance of retrieval design in LLM generalization pipelines.
% Last but not least, we present the significant improvement achieved by iterative learning, which can be up to 21.5\% compared to the results in the first-round generation.
% Given the expensive computational costs in iterative generation, we conduct a detailed analysis by investigating the relationships between LLMs generalization performance and the number of tokens LLMs process.
% Upon publication, we will release our code and new benchmarks, including annotation of oracle documents and ground-truth code solutions for each example, together with pools of documentation, to serve as a test-bed for future research on updated libraries and long-tail programming languages.

% It consists of four datasets, where two feature in updated libraries and two feature in long-tailed programming languages.


% On the one hand, public libraries are rapidly updated and new/varied programming languages are proposed to fit downstream applications.
% On the other hand, it is impractical to keep training LLM on library updates or new programming languages due to the limited data and high computational cost.

% Recent research has found the emergent abilities of LLM, where LLM exhibit exceptional performance on tasks they were not explicitly trained.


